Safe Spaces or Toxic Places? Content Moderation and Social Dynamics of Online Eating Disorder Communities

Social media platforms have become critical spaces for discussing mental health concerns, including eating disorders. While these platforms can provide valuable support networks, they may also amplify harmful content that glorifies disordered cognition and self-destructive behaviors. While social media platforms have implemented various content moderation strategies, from stringent to laissez-faire approaches, we lack a comprehensive understanding of how these different moderation practices interact with user engagement in online communities around these sensitive mental health topics. This study addresses this knowledge gap through a comparative analysis of eating disorder discussions across Twitter/X, Reddit, and TikTok. Our findings reveal that while users across all platforms engage similarly in expressing concerns and seeking support, platforms with weaker moderation (like Twitter/X) enable the formation of toxic echo chambers that amplify pro-anorexia rhetoric. These results demonstrate how moderation strategies significantly influence the development and impact of online communities, particularly in contexts involving mental health and self-harm.

==> scratch.tex <==
Online communities provide a vital space for socializing, sharing information, and receiving social and emotional  support~\cite{ellison2007benefits}, especially for individuals dealing with sensitive topics like body image and mental health. However, maintaining safe, welcoming, and inclusive online environment has proven challenging. Online communities that indoctrinate users into extreme ideologies~\cite{schmitz2022quantifying} or glorify self-harm~\cite{Goldenberg2022ncri} are especially challenging to moderate, as users often evade moderation through the use of coded language, insider jargon and intentional misspellings~\cite{chancellor2016thyghgapp,cobb2017not,bickham2024hidden}.
While some social media platforms have made progress in identifying and moderating online speech that violates community norms, such as hate speech and personal attacks~\cite{jhaver2019human,rajadesingan2020quick}, others have adopted a more laissez-faire approach.
These varied strategies for moderating online content, including discussions on sensitive mental health topics, have produced vastly different user experiences and engagement in online communities across platforms.



This paper examines online discussions of eating disorders on different social media platforms as a microcosm of mental health concerns.  
Eating disorders represent a serious mental health condition characterized by obsessive thoughts and unhealthy behaviors around food, eating, and body size. The condition, which includes anorexia, bulimia, and binge eating disorder, affects 24 million~\cite{vanHoeken2020review} people in the US 
and is among the deadliest of all mental health conditions,  with over 10,000 deaths each year in the US. 
The COVID-19 pandemic has amplified the disorder~\cite{nutley2021impact}, particularly among girls and young women~\cite{Hartman2022}. According to the CDC, the number of weekly visits to emergency rooms for adolescent girls struggling with eating disorders has doubled in 2021 compared to 2019~\cite{radhakrishnan2022pediatric}. 


Researchers have linked the rise in eating disorders to the proliferation of idealized body images in the media~\cite{becker2004television}, especially social media platforms like Instagram and Tiktok that promote the ``thin ideal'' and the ``muscular ideal''~\cite{fardouly2016social,marks2020pursuit,lavender2017men}. Exposure to idealized body images invites negative comparisons and pressure to conform to unrealistic beauty standards, which contributes to negative body image, a known risk factor for developing eating disorders~\cite{choukas2022perfectstorm}.


We argue that the relationship between social media and eating disorders is more complex and, in the absence of moderation, creates conditions that exacerbate them. First, social media search and recommendation algorithms may channel vulnerable individuals searching for weight loss and fitness advice to harmful content that promotes extreme dieting and over-exercising. Second, individuals may stumble upon pro-anorexia communities and influencers that glorify thinness and view anorexia as an aesthetic rather than a serious medical condition~\cite{Ging2018,wang2018social}. Such online spaces arguably provide support to individuals struggling with eating disorders, including a safe space to vent  and emotional validation~\cite{oksanen2016proanorexia,YeshuaKatz2013stigma}; however, they may ultimately harm them by normalizing disordered cognitions and delaying recovery~\cite{pater2016hunger,pater2017defining,chancellor2016recovery}.
Although pro eating disorder communities in the form of blogs and message forums have existed since the early days of the web~\cite{Ging2018}, social media has vastly expanded its reach. 


Social media platforms have taken disparate approaches to moderating content related to eating disorders. Platforms like Tiktok and Instagram restrict potentially harmful content. Searches for pro-anorexia terms like ``thin inspiration'' and ``proana'' return resources from health organizations instead. However, critics have argued that these efforts are insufficient and fail to detect when users deliberately obfuscate harmful content.\footnote{\url{https://counterhate.com/wp-content/uploads/2022/12/CCDH-Deadly-by-Design_120922.pdf}\label{note1}} %.pdf#page=44.12
Reddit has banned harmful forums, or subreddits, that glorify anorexia in 2018 and relies on community moderators to police conversations in eating disorders forums.
In contrast, Twitter does not forcefully moderate pro-anorexia speech~\cite{Sukunesan2021},  and as a result, content glorifying eating disorders and self-harm has proliferated on the platform even before the 2022 ownership change~\cite{Goldenberg2022ncri}. 
However, the link between community moderation, user engagement and eating disorders content has not been widely explored.

This study presents a comparative analysis of eating disorder discussions across Twitter, Reddit, and Tiktok. We collected posts from Tiktok and Twitter using the same set of search terms related to dieting, weight loss, body image concerns, and eating disorders, and we gathered relevant discussions from Reddit forums (i.e., subreddits) on similar themes. Our analysis reveals that users on all platforms discuss body image and eating disorder concerns, often integrating these topics into broader conversations about dieting. Users across platforms engage with online  communities in a similar manner, both venting, or expressing negative emotions, and receiving emotional support through positive replies.

However, among the three platforms, Twitter stands out for its toxicity. Semantically, content that glorifies anorexia and self harm proliferates on the site, but forms a cluster of interlinked topics, well separated from other discussions. By contrast, Tiktok content is more recovery-oriented, although it is more integrated within mainstream topics. Socially, users link within tight-knit communities on Twitter, forming echo chambers. In contrast, eating disorders communities on Reddit are integrated with other topics.

Our findings underscore the benefits of content moderation. Platforms with weaker moderation, like Twitter, enable harmful communities to flourish, creating echo chambers that amplify pro-anorexia rhetoric and ensnare even more vulnerable users.  This vicious spiral provides a plausible mechanism for the increase in content glorifying eating disorders on Twitter~\cite{Goldenberg2022ncri}. 


Social media can be especially damaging to body image during critical developmental periods when people learn to evaluate their appearance. Social platforms expose users to peers---a potent source of comparison~\cite{Festinger}---on a global scale. Furthermore, social media can propagate psychological distress through psychological contagion. Conditions like tics~\cite{olvera2021tiktok}, psychogenic illness~\cite{bartholomew2012mass}, and suicidality~\cite{gould2001suicide} have been shown to spread with media exposure. Effective moderation, such as adherence to suicide reporting guidelines, has been proven to mitigate harm~\cite{sumner2020adherence}. Understanding the interplay between online communities and moderation practices is crucial to minimizing social media’s negative impact on mental health and promoting recovery-oriented discussions.
